Oscillating photonic Bell state from a semiconductor quantum dot for quantum key distribution

An on-demand source of bright entangled photon pairs is desirable for quantum key distribution (QKD) and quantum repeaters. The leading candidate to generate entangled photon pairs is based on spontaneous parametric down-conversion (SPDC) in a non-linear crystal. However, there exists a fundamental trade-off between entanglement fidelity and efficiency in SPDC sources due to multiphoton emission at high brightness, which limits the pair extraction efficiency to 0.1% when operating at near-unity fidelity. Quantum dots in photonic nanostructures can in principle overcome this trade-off; however, the quantum dots that have achieved entanglement fidelities on par with SPDC sources (99%) have poor pair extraction efficiencies of 0.01%. Here, we demonstrate a 65-fold increase in the pair extraction efficiency compared to quantum dots with equivalent peak fidelity from an InAsP quantum dot in a photonic nanowire waveguide. We measure a raw peak concurrence and fidelity of 95.3% $\pm$ 0.5% and 97.5% $\pm$ 0.8%, respectively. Finally, we show that an oscillating two-photon Bell state generated by a semiconductor quantum dot can be utilized to establish a secure key for QKD, alleviating the need to remove the quantum dot energy splitting of the intermediate exciton states in the biexciton-exciton cascade.

==> NDraft.tex <==
\newcommand{\deltaleak}{\delta_{\text{leak}}}
\renewcommand{\Tr}[1]{\textrm{Tr}\left [ #1 \right ]}        %
\newcommand{\ntimebin}{{n_{\textrm{bin}}}}
\newcommand{\nrounds}{{n_{\textrm{round}}}}
\newcommand{\vecA}{{\vec{i}}} %
\newcommand{\vecB}{{\vec{j}}} %
\newcommand{\vecAn}{{\vec{n}}} %
\newcommand{\vecBn}{{\vec{m}}} %
\newcommand{\vecASingle}[1]{{\vec{i}_{#1}}} %
\newcommand{\vecBSingle}[1]{{\vec{j}_{#1}}} %


In this supplement, we describe a general method to calculate secret key rates for entanglement-based (EB) QKD experiments that use fast detectors. The idea is to break each round of the protocol into $\ntimebin$ time-bins where the detectors record the click patterns in each time-bin. We then use this to calculate key rates for the QD source with non-zero FSS.

In our security proof, we assume that the threshold detectors used have no memory effects (detector dead times, afterpulsing, etc.), and all detectors have the same detection efficiency.
Any security proof for independent and identically distributed (iid) states can be lifted to a security proof for general states via the quantum de Finetti theorem \cite{renner2007symmetry} or the postselection technique \cite{christandl2009postselection}\DIFdelbegin \DIFdel{. 
Thus, }\DIFdelend \DIFaddbegin \DIFadd{, which are asymptotically tight. 
As we only consider asymptotic key rates, we can thus }\DIFaddend without loss of generality \DIFdelbegin \DIFdel{, we can }\DIFdelend assume that Alice and Bob's shared state is iid i.e. $\rho_{A^{\nrounds}B^{\nrounds}} = \rho_{AB}^{\otimes \nrounds}$, where $\nrounds$ is \DIFdelbegin \DIFdel{the }\DIFdelend \DIFaddbegin \DIFadd{a large }\DIFaddend number of protocol rounds. In the rest of this supplement we focus on proving security for these iid states.

\subsubsection{QKD Protocol Steps}

Here we outline the steps in a generic time-resolved entanglement-based (EB) protocol with $\nrounds$ rounds.
\begin{enumerate}
    \item \label{QKDprotocol:transm} \textbf{Signal transmission:} Eve prepares optical states $\rho_{AB}$ to send to Alice and Bob.
    \item \textbf{Measurement:} Alice and Bob each have sets of POVM elements $\{\Gamma^{A}_{\vecA}\}$ and $\{\Gamma^{B}_{\vecB}\}$. Here, the elements $i_{k}$ and $j_{k}$ of the vectors $\vecA$ and $\vecB$ represent the click patterns observed in time-bin $k$.
\end{enumerate}
After repeating the above steps $\nrounds$ times, we proceed to the next part of the protocol.
\begin{enumerate}[resume]
    \item \DIFdelbegin %
\DIFdelend \DIFaddbegin \label{QKDprotocol:accTest} \DIFaddend \textbf{Acceptance testing:} Alice and Bob randomly choose a subset of the rounds for testing. For the rounds chosen for testing, they both publicly announce their measurement results $\vecA$ \DIFdelbegin \DIFdel{, }\DIFdelend \DIFaddbegin \DIFadd{and }\DIFaddend $\vecB$ to form a distribution of the frequency of events. They then check if this frequency distribution belongs to the acceptance set agreed upon before running the protocol. If it does, they proceed with the protocol after discarding the test results. Otherwise, they abort.
    \item \label{QKDprotocol:announce} \textbf{Announcements and sifting:} Alice and Bob make announcements over the authenticated classical channel. They sift the non-tested data based on the announcements made i.e. they choose a subset of signal and measurement data to keep and discard the rest based on the announcements.
    \item \label{QKDprotocol:keyMap} \textbf{Key Map:} Alice uses her measurement results $\vecA$ as well as the announcements to map her data into a key string $x$. This is called the raw key.
    We assume here that the key is a bit string for simplicity, but all the steps can be applied more generally.
    \item \label{QKDprotocol:protocolStepErrorCorr} \textbf{Error Correction:} Alice and Bob then perform error correction over the authenticated classical channel to make Bob's measurement outcomes $\vecB$ match with Alice's bit string $x$. We denote the data communicated per key bit to Eve in this process as $\deltaleak$.
    \item \textbf{Privacy Amplification:} Alice and Bob produce their final secret key by applying an appropriate hash function on the raw key (Theorem 5.5.1 of \cite{renner2008security}).
\end{enumerate}

\subsubsection{Key rate calculation}

\begin{itemize}
    \item The secret key rate in the asymptotic limit in the iid case can be found using the Devetak-Winter formula \cite{devetak2005distillation}: $R = H(Z\vert E)-\deltaleak$ where $Z$ is the key register, $E$ is Eve's register, and $\deltaleak$ is the number of bits per round leaked to Eve during Step \ref{QKDprotocol:protocolStepErrorCorr} of the protocol.
    \begin{itemize}
            \item A lower bound for the key rate can be found by minimising $H(Z\vert E)$ over Eve's marginal states consistent with the observed statistics.
            \item Following \cite{coles2016numerical,winick2018reliable}, this minimisation can be reformulated as an SDP
            \begin{equation} \label{eq:mainKeyRate}
                \begin{aligned}
                    R = \underset{\rho_{AB}}{\textrm{min }} &D\left(\mathcal{G}\left(\rho_{AB}\right)\vert\vert\mathcal{Z}\left(\mathcal{G}\left(\rho_{AB}\right)\right)\right) - \delta_\textrm{leak} \\
                    \textrm{s.t. } &\Tr{\left(\Gamma_{\vecA}\otimes \Gamma_{\vecB}\right)\rho_{AB}} = p_{\vecA \vecB} \quad\quad\forall \vecA,\vecB\\
                    &\rho_{AB} \geq 0,
                \end{aligned}
            \end{equation}
            where $A$ and $B$ are Alice and Bob's registers. The observed statistics $p_{\vecA\vecB}$ is the probability of Alice and Bob observing outcomes $\vecA$ and $\vecB$ respectively. \DIFaddbegin \DIFadd{Note that in phrasing the optimisation problem in this way, we have implicitly chosen a point acceptance set (Step \ref{QKDprotocol:accTest} of protocol steps) to be exactly the statistics from the honest implementation as we only consider the asymptotic limit.
            }\DIFaddend \item Here, the relative entropy $D\left(\mathcal{G}\left(\rho_{AB}\right)\vert\vert\mathcal{Z}\left(\mathcal{G}\left(\rho_{AB}\right)\right)\right)-\deltaleak$ is the objective function where $\mathcal{G}$ is a map that represents the protocol (including announcements), and $\mathcal{Z}$ is a map that can be constructed from the key map. Since we do not use most of the specific details of these maps, we abstract the objective function as $f(\rho_{AB})$. For more details, see \cite{winick2018reliable, coles2016numerical}.
        \end{itemize}
        \item The aim is to reduce this to a problem that is numerically tractable. There are two obstacles to doing this.
        \begin{itemize}
            \item The first is that each time-bin has an infinite-dimensional Fock space associated with it. This is a well-studied problem in QKD \cite{fung2011universal,gittsovich2014squashing,li2020improving,upadhyaya2021dimension}. Any of these methods can be used to reduce the problem to solving finite-dimensional SDPs in each time-bin. 
            \item The dimension of the space after this process is still large due to the multiple time-bins. Thus, we will simplify Eq. (\ref{eq:mainKeyRate}) to a minimization on each time-bin individually to obtain a ``time-resolved key rate''.
        \end{itemize}
    \end{itemize}

    \subsubsection{Time-resolved key rate}

    \begin{itemize}
        \item Since we assume that the threshold detectors have no memory effects, each of Alice and Bob's POVM elements can be \DIFdelbegin \DIFdel{modelled }\DIFdelend \DIFaddbegin \DIFadd{modeled }\DIFaddend as $\Gamma_{\vec{i}}=\bigotimes_{k=1}^\ntimebin\Gamma_{i_k}$.
        \begin{itemize}
            \item For threshold detectors such as the SNSPDs, $\Gamma_{i_k}$ is block diagonal in the total number of photons in time-bin $k$ i.e.
            \begin{equation}
                \Gamma_{i_k}=\bigoplus_{n_k=0}^\infty\Gamma_{i_k}^{n_k}.
            \end{equation}
            \item Thus, the POVM elements $\Gamma_{\vec{i}}$ are block-diagonal as
            \begin{equation}
                \Gamma_{\vec{i}} = \bigoplus_{\vec{n}}  \Gamma^{n_1}_{i_1}\otimes  \Gamma^{n_2}_{i_2} \otimes \ldots \otimes \Gamma^{n_\ntimebin}_{i_\ntimebin}.
            \end{equation}
            \item As a result, we can without loss of generality (see for instance, Observation 8 from \cite{gittsovich2014squashing}) assume that Alice and Bob's joint state has the same block-diagonal structure
            \begin{equation}
                \rho_{AB} = \bigoplus_{\vecAn, \vecBn} \rho_{AB}^{\vecAn\vecBn},
            \end{equation}
            where $\rho_{AB}^{\vecAn\vecBn}$ are sub-normalised states.
        \end{itemize}
        \item Following Eq. (D.9) from \cite{li2020application}, we can exploit the block-diagonal structure in the state to write $f(\rho_{AB}) = \sum_{\vecAn,\vecBn} f(\rho_{AB}^{\vecAn\vecBn})$, where $f(\rho_{AB})$ is the objective function of the SDP in Eq. (\ref{eq:mainKeyRate}). Thus, $R\geq \sum_{\vecAn,\vecBn} R^{\vecAn\vecBn}$ where 
        \begin{equation} \label{eq:BlockKeyRate}
            \begin{aligned}
                R^{\vecAn\vecBn} = \underset{\rho_{AB}}{\textrm{min }} &f\left(\rho_{AB}^{\vecAn\vecBn}\right)\\
                \textrm{s.t. } &\Tr{\left(\Gamma_{\vecA}\otimes \Gamma_{\vecB}\right)\rho_{AB}} = p_{\vecA \vecB} \quad\quad\forall \vecA,\vecB\\
                &\rho_{AB} \geq 0\\
                &\rho_{AB} = \bigoplus_{\vecAn, \vecBn} \rho_{AB}^{\vecAn\vecBn}.
            \end{aligned}
        \end{equation}
        Since each $R^{\vecAn\vecBn}$ is positive, taking finitely many of these terms is sufficient to lower bound the key rate. In particular, we consider those terms where all but one time-bin has no photons on each of Alice and Bob's sides.
        \begin{itemize}
            \item Note that $\rho_{AB}^{\vecAn_{k_c}\vecBn_{l_c}}=\rho_{AB}^{n_{k_c}m_{l_c}}\bigotimes_{k\neq k_c, l\neq l_c}\ketbra{0}_k\otimes\ketbra{0}_l$ where $k_c$ and $l_c$ are the time-bins with photons on Alice and Bob's side respectively.
        \end{itemize}
        \item If the detection efficiency of all detectors is identical, it is sufficient to prove security for lossless detectors instead \cite{lutkenhaus1999estimates} \DIFaddbegin \DIFadd{by considering loss to be a part of the channel}\DIFaddend . In this case, for all Alice's events $\vecASingle{k_c}$ that have detection events in just time-bin $k_c$, 
        $\Gamma_{\vecASingle{k_c}} = \Gamma_{i_{k_{c}}}\bigotimes_{k\neq k_{c}} \ketbra{0}_{k}$. Similarly, $\Gamma_{\vecBSingle{l_c}} = \Gamma_{j_{l_{c}}}\bigotimes_{l\neq l_{c}} \ketbra{0}_{l}$ for all Bob's events $\vecBSingle{l_c}$ that have detection events in just time-bin $l_c$.
        Thus, 
        \begin{align}
            \nonumber \Tr{\left(\Gamma_{\vecASingle{k_c}}\otimes \Gamma_{\vecBSingle{l_c}}\right)\rho_{AB}} &= \Tr{\left(\Gamma_{\vecASingle{k_c}}\otimes \Gamma_{\vecBSingle{l_c}}\right)\sum_{n_{k_c},m_{l_c}=0}^\infty\rho_{AB}^{\vecAn_{k_c}\vecBn_{l_c}}}\\
            &= \Tr{\left(\Gamma_{i_{k_c}}\otimes \Gamma_{j_{l_c}}\right)\rho_{AB}^{{k_c}{l_c}}},\label{eq:QKDDetectorSimpllify}
        \end{align}
        where $\vecAn_{k_c}$ ($\vecBn_{l_c}$) are vectors where all but the $k_c$ ($l_c$) entry is 0, and $\rho_{AB}^{{k_c}{l_c}} = \sum_{n_{k_c},m_{l_c}=0}^\infty \rho_{AB}^{n_{k_c}m_{l_c}}$. Note that the right hand side of Eq. (\ref{eq:QKDDetectorSimpllify}) is described in terms of operators that act on the space for a single time-bin $k_c$, $l_c$ for Alice and Bob respectively.
        \begin{itemize}
            \item For all events $\vecA$, $\vecB$ with clicks in more than one time-bin, $\Tr{\left(\Gamma_{\vecA}\otimes \Gamma_{\vecB}\right)\rho_{AB}^{\vecAn_{k_c}\vecBn_{l_c}}} = 0$.
        \end{itemize}
        \item Additionally, we define the function $g\left(\rho_{AB}^{{k_c}{l_c}}\right) \coloneqq \sum_{n_{k_c},m_{l_c}=0}^\infty f\left(\rho_{AB}^{\vecAn_{k_c}\vecBn_{l_c}}\right)$ acting on the space for a single time bin for Alice and Bob.
        Thus, the SDP in Eq. (\ref{eq:BlockKeyRate}) can be simplified as
        \begin{equation} \label{eq:timeResolvedKeyRate}
            \begin{aligned}
                R^{k_c l_c} = \underset{\rho_{AB}^{{k_c}{l_c}}}{\textrm{min }} &g\left(\rho_{AB}^{{k_c}{l_c}}\right)\\
                \textrm{s.t. } &\Tr{\left(\Gamma_{i_{k_c}}\otimes \Gamma_{j_{l_c}}\right)\rho_{AB}^{{k_c}{l_c}}} = p_{\vecASingle{k_c} \vecBSingle{l_c}} \quad\quad\forall \vecASingle{k_c},\vecBSingle{l_c}\\
                &\rho_{AB}^{{k_c}{l_c}} \geq 0.
            \end{aligned}
        \end{equation}
        \DIFaddbegin \item \DIFaddend We define $r(\tau)=\frac{\sum_{\abs{k_c-l_c}=\tau}R^{k_c l_c}}{\Tr{\rho_{AB}^{\tau}}}$ to be the time-resolved key rate where $\rho_{AB}^{\tau} = \sum_{\abs{k_c-l_c}=\tau} \rho_{AB}^{{k_c}{l_c}}$\DIFaddbegin \DIFadd{.
        }\DIFaddend Thus, we have simplified the key rate SDP in Eq. (\ref{eq:mainKeyRate}) to the time-resolved key rate SDPs described in Eq. (\ref{eq:timeResolvedKeyRate}) which act on the spaces corresponding to a single time-bin $k_c$, $l_c$ for Alice and Bob respectively.
        \item The time-resolved key rate SDPs described in Eq. (\ref{eq:timeResolvedKeyRate}) are still infinite-dimensional. As discussed above, any of the techniques from \cite{fung2011universal,gittsovich2014squashing,li2020improving,upadhyaya2021dimension} to reduce this to a finite-dimensional optimisation can be used to obtain lower bounds on the time-resolved key rate. \DIFaddbegin \DIFadd{For the purposes of the example we consider in Section \ref{appSec:QKDPoPExp}, we use the dimension reduction method from \mbox{%
\cite{upadhyaya2021dimension}}\hskip0pt%
.
}\DIFaddend \end{itemize}

\subsubsection{Proof-of-principle experiment} \DIFaddbegin \label{appSec:QKDPoPExp}
\DIFaddend 

So far, we have described a generic framework to compute key rates with fast detectors \DIFaddbegin \DIFadd{i.e. detectors with low timing jitter and dead times to resolve subsequent time-bins with independent detection events}\DIFaddend . We now describe how we used this framework to obtain the plots in Figure \ref{fig:qkd_keyrate}, which clearly demonstrate the utility of a QD with non-zero FSS. \DIFaddbegin \DIFadd{Note that in the proof-of-principle experiment, we consider the case where only single-click events, i.e. a click only in a single detector time-bin in each protocol round for Alice and Bob each. As we expect our source to primarily send out single-photon states to Alice and Bob each, this would be close to what we expect to observe in a real experiment.
}\DIFaddend \begin{itemize}
    \item We consider a polarisation-based 6-state protocol \cite{bruss1998optimal} where both Alice and Bob measure their state in 3 conjugate polarisation bases which we term the `X', `Y' and `Z' bases. We set the probability of measuring in the Z-basis to be $\sqrt{0.99}$ each. After testing, they announce their basis data and discard all signals not in the Z-basis. Alice then maps single-clicks in the Z-basis into bits. Finally, they do error correction and privacy amplification.
    \item For the key rate calculation, we simulate the observations we expect to see from the characterized nanowire QD entangled photon source.
    \DIFdelbegin \DIFdel{For simplicity, we assume that there are only single-click events. }\DIFdelend \DIFaddbegin \begin{itemize}
        \item \DIFaddend We use the dimensional reduction method \cite{upadhyaya2021dimension} to construct finite-dimensional SDPs from Eq. (\ref{eq:timeResolvedKeyRate}) \DIFdelbegin \DIFdel{. }\DIFdelend \DIFaddbegin \DIFadd{which allows us to consider projections of measurments and states in a subspace only. For this, we need the weight $W = \Tr{\Pi_1 \rho^{k_c l_c}\Pi_1}$ outside the projected subspace. }\DIFaddend Thus, the time-resolved key rate can be lower bounded by the solution to the following finite-dimensional SDP:
        \begin{equation}
            \begin{aligned}
                R^{k_c l_c} \geq \underset{\rho_{AB}^{11}}{\textrm{min }} &g\left(\rho_{AB}^{11}\right)\\
                \textrm{s.t. } &p_{\vecASingle{k_c} \vecBSingle{l_c}}-W\leq \Tr{\left(\Gamma_{i_{k_c}}^1\otimes \Gamma_{j_{l_c}}^1\right)\rho_{AB}^{11}} \leq p_{\vecASingle{k_c} \vecBSingle{l_c}} \quad\quad\forall \vecASingle{k_c},\vecBSingle{l_c}\\
                &\rho_{AB}^{11} \geq 0,
            \end{aligned}
        \end{equation}
        where $\Gamma^1 = \Pi_1 \Gamma \Pi_1$ is the projection of the POVM elements into the single-photon subspace $\Pi_1$. \DIFdelbegin \DIFdel{Here, $W = \Tr{\Pi_1 \rho^{k_c l_c}\Pi_1}$ which }\DIFdelend \DIFaddbegin \DIFadd{Note that since the POVM elements commute with our chosen projection, we have used the tighter Eq. (49) from \mbox{%
\cite{upadhyaya2021dimension}}\hskip0pt%
.
    }\end{itemize}
    \DIFadd{Here, the weight outside the subspace $W$ }\DIFaddend can be estimated from the multi-click events (see for e.g.- \cite{narasimhachar2011study,li2020improving, nahar2023imperfect} for some protocol-dependent techniques to do this). In our case, since we have \DIFdelbegin \DIFdel{no multi-click }\DIFdelend \DIFaddbegin \DIFadd{assumed to observe only single-click }\DIFaddend events, this can be calculated exactly to be $W=0$. Thus, the time-resolved key rate SDP simplifies to numerically optimising an SDP in the qubit space.
    \item Additionally since we are performing the 6-state experiment, we have a tomographically complete set of measurements on the qubit space. Thus, the state $\rho_{AB}^{11}$ can be determined exactly from the observations for each time-bin. As a result, we can compute the time-resolved key rates $r(\tau)$ by simply computing the objective functions for the qubit density matrix for the time-bins. \DIFaddbegin \DIFadd{So no SDP optimisations are required for our simple example.
    }\DIFaddend \item Finally, \DIFdelbegin \DIFdel{to obtain the blue curve in Figure \ref{fig:qkd_keyrate}, we optimise }\DIFdelend \DIFaddbegin \DIFadd{as described in Supplementary note \ref{supp-sec:time-resolved_ent_fidelity}, the actual entangled photon pair does not rotate in the $HH-VV$ plane as described by Eq. (\ref{eq:bellstate-fss}). Thus, our initial key map consisting of $H$ and $V$ polarisations might not be optimal. We instead run an optimisation }\DIFaddend over all choices of conjugate polarisation bases to \DIFdelbegin \DIFdel{take into account the fact that the quantum dot does not actually rotate in the plane spanned by $HH$ and $VV$. This }\DIFdelend \DIFaddbegin \DIFadd{measure in. We use the result of this optimisation to create the blue curve in Fig. \ref{fig:qkd_keyrate}. Practically, this }\DIFaddend can be implemented in the protocol by adding appropriate waveplates before Alice and Bob's entire measurement setup.
\end{itemize}

==> QKD.tex <==
In this paper, we aimed to show that the fine structure splitting of quantum dots was not a hindrance to quantum information processing tasks. As an example, we compute the key rates for a QKD setup under the following assumptions:
\begin{enumerate}
    \item We work in the \textit{asymptotic} limit with infinitely many rounds of the QKD protocol.
    \item We assume that the state coming into Alice and Bob's labs live in the \textit{qubit} space i.e. Alice and Bob receive a single photon each.
    \item We assume that we can perform error correction in the Shannon limit.
    \item We assume that the detectors are ideal.
\end{enumerate}
Additionally, any security proof for independent and identically distributed (iid) states can be lifted to a security proof for general states via the quantum de Finetti theorem \cite{renner2007symmetry} or the postselection technique \cite{christandl2009postselection}. Thus, without loss of generality we can assume that Alice and Bob's shared state is iid.

In the 6-state protocol, Alice and Bob perform the following protocol steps:
\begin{enumerate}
    \item \textbf{Transmission:} Eve prepares qubits to send to Alice and Bob.
    \item \textbf{Measurement:} Alice and Bob randomly choose one of the $H$/$V$, $A$/$D$, and $R$/$L$ bases to measure in for each round of the protocol. In addition, they also measure the time delay between their detection events. Under the qubit assumption, these are a tomographically complete set of measurements.
    \item \textbf{Testing:} They choose a random subset of the data and announce their measurement results.
    Thus, under the asymptotic iid assumptions, we can tomographically reconstruct the shared state between Alice and Bob for each time delay.
    \item \label{protocol:annAndSift} \textbf{Announcements and sifting:} Alice and Bob announce their measurement basis, and discard all data except where they both measured in the $H$/$V$ basis.
    \item \textbf{Key map:} Amongst all remaining data, Alice maps $H$ to $0$, and $V$ to $1$ to generate the raw key. We denote the register storing the raw key by $X$.
    \item \textbf{Error correction:} Alice and Bob perform error correction to make Bob's data to match the raw key. The data communicated in this step can be bound in the Shannon limit by $H(X\vert Y)$ where $Y$ denotes the register storing Bob's classical data prior to error correction.
    \item \textbf{Privacy amplification:} Alice and Bob produce their final secret key by applying an appropriate hash function on the raw key (Theorem 5.5.1 of \cite{renner2008security}).
\end{enumerate}

A lower bound on the number of secret bits per pulse sent can be found using the Devetak-Winter key rate formula \cite{devetak2005distillation}
\begin{equation}
    R = H(Z\vert E) -H(Z\vert Y),
\end{equation}
where $E$ is Eve's quantum register.
Following \cite{coles2016numerical,winick2018reliable} the Devetak-Winter key rate formula can be reformulated as a function of $\rho_{AB}$
\begin{equation} \label{eq:keyRate}
    R(\rho_{AB}) = D\left(\mathcal{G}\left(\rho_{AB}\right)\vert\vert\mathcal{Z}\left(\mathcal{G}\left(\rho_{AB}\right)\right)\right)-H(Z\vert Y),
\end{equation}
where $\mathcal{G}$ is a map that represents the measurement and announcement steps of the protocol, and $\mathcal{Z}$ is a map that can be constructed from the key map step of the protocol.

Alice and Bob's shared state $\rho_{AB}(\tau)$ can be determined in the testing step of the protocol for each time delay $\tau$. Thus, we can calculate the time-resolved key rate $R(\tau)$ by performing error correction and privacy amplification independently for each $tau$. The lifetime-weighted key rate can then be calculated by weighting $R(\tau)$ with the probability of the quantum dot excitation producing time delay $\tau$.

For the purposes of our demonstration, we choose the probability of Alice and Bob choosing the $H$/$V$ basis to be $\sqrt{0.99}$. Thus, the probability of a signal being discarded in step \ref{protocol:annAndSift} of the protocol is 0.01. This upper bounds the key rate for an ideal state at 0.99.
For the black curve in Figure \ref{fig:qkd_keyrate}, we compute key rates for $\ket{\psi(\tau)}$ as defined in Eq. (\ref{eq:bellstate-fss}). Thus, we input $\rho_{AB}(\tau) = \ket{\psi(\tau)}\!\bra{\psi(\tau)}$ in Eq. (\ref{eq:keyRate}) to get the time-resolved key rates. We observe that this exactly achieves the upper bound 0.99.
Similarly, we use the dephasing-free model to obtain the red curve in Figure \ref{fig:qkd_keyrate}.

To obtain the blue curve in Figure \ref{fig:qkd_keyrate}, we first get the reconstructed density matrix for the quantum dot $\rho'_{AB}(\tau)$. We then optimise over all rotations acting indpendently on Alice and Bob's parts of the state to take into account the fact that the quantum dot does not actually rotate in the plane spanned by $HH$ and $VV$. This can be implemented in the protocol by adding appropriate waveplates before Alice and Bob's entire measurement setup. This rotated density matrix forms the input $\rho_{AB}$ into the time-resolved key rate in Eq. (\ref{eq:keyRate}).

We acknowledge that these assumptions are not physically motivated. Additionally, the parameter regimes chosen, and protocol construction are not optimal for finite-size key rates. Thus, further work must be done to prove security without making these simplifying assumptions.
However, we emphasise that the key rates we compute from this are representative of the key rate of an actual QKD experiment with fine structure splitting. Thus, fine structure splitting would not be a hindrance to QKD with fast detectors.
